Separation of Neural Drives to Muscles from Transferred Polyfunctional Nerves using Implanted Micro-electrode Arrays

Following limb amputation, neural signals for limb functions persist in the residual peripheral nerves. Targeted muscle reinnervation (TMR) allows to redirected these signals into spare muscles to recover the neural information through electromyography (EMG). However, a significant challenge arises in separating distinct neural commands redirected from the transferred nerves to the muscles. Disentangling overlapping signals from EMG recordings remains complex, as they can contain mixed neural information that complicates limb function interpretation. To address this challenge, Regenerative Peripheral Nerve Interfaces (RPNIs) surgically partition the nerve into individual fascicles that reinnervate specific muscle grafts, isolating distinct neural sources for more precise control and interpretation of EMG signals. We introduce a novel biointerface that combines TMR surgery of polyvalent nerves with a high-density micro-electrode array implanted at a single site within a reinnervated muscle. Instead of surgically identifying distinct nerve fascicles, our approach separates all neural signals that are re-directed into a single muscle, using the high spatio-temporal selectivity of the micro-electrode array and mathematical source separation methods. We recorded EMG signals from four reinnervated muscles while volunteers performed phantom limb tasks. The decomposition of these signals into motor unit activity revealed distinct clusters of motor neurons associated with diverse functional tasks. Notably, our method enabled the extraction of multiple neural commands within a single reinnervated muscle, eliminating the need for surgical nerve division. This approach not only has the potential of enhancing prosthesis control but also uncovers mechanisms of motor neuron synergies following TMR, providing valuable insights into how the central nervous system encodes movement after reinnervation.

==> MU-tab.tex <==

\begin{tabular}{@{}l
>{\columncolor[HTML]{E1E4E9}}l 
>{\columncolor[HTML]{E1E4E9}}l 
>{\columncolor[HTML]{E1E4E9}}l ll@{}}
\toprule
\multicolumn{1}{|l|}{\textbf{Task}} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}l@{}}\# Total MUs\end{tabular}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}l@{}}\# MUs in \\ 100\% of reps\end{tabular}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}c@{}}\# MUs in \\ \textgreater{}70\% of reps\end{tabular}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}l@{}}\# Indep MU\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}\# MU with\\ satellite \\ potentials\end{tabular}}} \\ \midrule
\multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in pectoralis minor (TMR1)}} \\ \midrule
\multicolumn{1}{|l|}{Wrist Flexion} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}14.28} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}40.00} &
  \multicolumn{1}{l|}{4} \\ \midrule
\multicolumn{1}{|l|}{Pinky Flexion} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}42.85} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Pinky Abduction} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}8} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}8} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Intrinsic} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}42.85} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Tripod} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}9} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}9} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}66.66} &
  \multicolumn{1}{l|}{2} \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{C3C9D4}\textbf{Median nerve in pectoralis major pars abdominalis (TMR2)}} \\ \midrule
\multicolumn{1}{|l|}{Pronation} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{-} \\ \midrule
\multicolumn{1}{|l|}{Thumb Opposition} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}66.66} &
  \multicolumn{1}{l|}{-} \\ \midrule
\multicolumn{1}{|l|}{Flexion of Fingers} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{-} \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in biceps short head (TMR3)}} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}80.00} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Thumb + Intrinsic} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Flexion of Fingers} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}80.00} &
  \multicolumn{1}{l|}{4} \\ \midrule
\multicolumn{1}{|l|}{Pinky Flexion} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}66.66} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Tripod} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}75.00} &
  \multicolumn{1}{l|}{2} \\ \midrule
\multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in pectoralis minor (TMR4)}} \\ \midrule
\multicolumn{1}{|l|}{Pronation} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}33.33} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{-} \\ \midrule
\multicolumn{1}{|l|}{Pinky Flexion} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}50.00} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Pinky Abduction} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}0.00} &
  \multicolumn{1}{l|}{2} \\ \midrule
\multicolumn{1}{|l|}{Thumb Abduction} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}100.00} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Intrinsic} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}66.66} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Radial nerve in latissimus dorsi (TMR5)}} \\ \midrule
\multicolumn{1}{|l|}{Wrist Extension} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}100.00} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Wrist Supination} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}0.00} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Index Extension} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}20.00} &
  \multicolumn{1}{l|}{3} \\ \midrule
\multicolumn{1}{|l|}{Pinky Extension} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}40.00} &
  \multicolumn{1}{l|}{4} \\ \midrule
\multicolumn{1}{|l|}{Thumb Extension} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}100.00} &
  \multicolumn{1}{l|}{1} \\ \midrule
\multicolumn{1}{|l|}{Extension of Fingers} &
\multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}0.00} &
  \multicolumn{1}{l|}{2} \\ \bottomrule
\end{tabular}%
}




% \begin{tabular}{@{}l
% >{\columncolor[HTML]{E1E4E9}}l 
% >{\columncolor[HTML]{E1E4E9}}l 
% >{\columncolor[HTML]{E1E4E9}}l ll@{}}
% \toprule
% \multicolumn{1}{|l|}{\textbf{Task}} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}l@{}}\# MUs in \\ 100\% of reps\end{tabular}}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}c@{}}\# MUs in \\ \textgreater{}70\% of reps\end{tabular}}} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}\textbf{\begin{tabular}[c]{@{}l@{}}\# Indepndent MU\\ (\# Shared MU)\end{tabular}}} &
%   \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# MUs in\\  \textless 70\% of reps\end{tabular}}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}\# MU with\\ satellite \\ potentials\end{tabular}}} \\ \midrule
% \multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in Pectoralis Minor (TMR1)}} \\ \midrule
% \multicolumn{1}{|l|}{Wrist Flexion} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1 (6)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Ulnar Deviation} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5 (2)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{4} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Flexion} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4 (4)} &
%   \multicolumn{1}{l|}{4} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Abduction} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}8} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4 (4)} &
%   \multicolumn{1}{l|}{2} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Intrinsic} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}7} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3 (4)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Tripod} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}9} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6 (3)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{2} \\ \midrule
% \multicolumn{6}{c}{\cellcolor[HTML]{C3C9D4}\textbf{Median nerve in Pectoralis Major pars abdominalis (TMR2)}} \\ \midrule
% \multicolumn{1}{|l|}{Pronation} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1(1)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{-} \\ \midrule
% \multicolumn{1}{|l|}{Thumb Opposition} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2(1)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{-} \\ \midrule
% \multicolumn{1}{|l|}{Flexion of Fingers} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1(1)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{-} \\ \midrule
% \multicolumn{6}{c}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in Biceps SHort Head (TMR3)}} \\ \midrule
% \multicolumn{1}{|l|}{Ulnar Deviation} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5(1)} &
%   \multicolumn{1}{l|}{2} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Thumb + Intrinsic} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2(1)} &
%   \multicolumn{1}{l|}{2} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Flexion of Fingers} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4(1)} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{4} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Flexion} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6(1)} &
%   \multicolumn{1}{l|}{4} &
%   \multicolumn{1}{l|}{5} \\ \midrule
% \multicolumn{1}{|l|}{Tripod} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2(2)} &
%   \multicolumn{1}{l|}{2} &
%   \multicolumn{1}{l|}{2} \\ \midrule
% \multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Ulnar nerve in Pectoralis Minor (TMR4)}} \\ \midrule
% \multicolumn{1}{|l|}{Pronation} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1 (2)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Ulnar Deviation} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1 (1)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{-} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Flexion} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4 (2)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Abduction} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}- (1)} &
%   \multicolumn{1}{l|}{3} &
%   \multicolumn{1}{l|}{2} \\ \midrule
% \multicolumn{1}{|l|}{Thumb Abduction} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3 (-)} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Intrinsic} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}3} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2 (1)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{6}{|c|}{\cellcolor[HTML]{C3C9D4}\textbf{Radial nerve in Latissimus Dorsi (TMR5)}} \\ \midrule
% \multicolumn{1}{|l|}{Wrist Extension} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4 (-)} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Wrist Supination} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}- (1)} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Index Extension} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}1 (4)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{3} \\ \midrule
% \multicolumn{1}{|l|}{Pinky Extension} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}5} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2 (3)} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{4} \\ \midrule
% \multicolumn{1}{|l|}{Thumb Extension} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}4} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}6 (-)} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} \\ \midrule
% \multicolumn{1}{|l|}{Extension of Fingers} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}2} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}-} &
%   \multicolumn{1}{l|}{\cellcolor[HTML]{E1E4E9}- (2)} &
%   \multicolumn{1}{l|}{-} &
%   \multicolumn{1}{l|}{2} \\ \bottomrule
% \end{tabular}%
% }

==> TMR1_cluster_13.tex <==
\begin{tabular}{@{}|cccccc|@{}}
\toprule
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{MFR [\SI{}{\hertz}]} &
  \multicolumn{1}{c|}{Rec Th [\%]} &
  \multicolumn{1}{c|}{Normalised MUAP area} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}MUAP  peak-to-peak\\ Amplitude [\SI{}{\micro\volt}]\end{tabular}} &
  MUAP Size [\SI{}{\micro\volt \milli\second}] \\ \midrule
\multicolumn{6}{|l|}{\textbf{TMR1}} \\ \midrule
\multicolumn{1}{|c|}{Corr $\geq 0.5$} &
  \multicolumn{1}{c|}{12.935 $\pm$ 2.733} &
  \multicolumn{1}{c|}{6.148 $\pm$ 2.067} &
  \multicolumn{1}{c|}{0.032 $\pm$ 0.043} &
  \multicolumn{1}{c|}{27.068 $\pm$ 26.790} &
  53.637 $\pm$ 45.818 \\ \midrule
\multicolumn{1}{|c|}{Corr $< 0.5$} &
  \multicolumn{1}{c|}{11.796 $\pm$ 3.725} &
  \multicolumn{1}{c|}{8.502 $\pm$ 3.277} &
  \multicolumn{1}{c|}{0.028 $\pm$ 0.046} &
  \multicolumn{1}{c|}{54.205 $\pm$ 75.792} &
  106.220 $\pm$ 148.856 \\ \midrule
\multicolumn{1}{|c|}{P-Value ($<$ 0.05)} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}0.006} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}$<$ 0.05} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}$<$ 0.05} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}0.001} &
  0.164 \\ \midrule
\multicolumn{6}{|l|}{\textbf{TMR3}} \\ \midrule
\multicolumn{1}{|c|}{Corr $\geq 0.5$} &
  \multicolumn{1}{c|}{11.949 $\pm$ 1.497} &
  \multicolumn{1}{c|}{3.939 $\pm$ 1.212} &
  \multicolumn{1}{c|}{0.044 $\pm$ 0.057} &
  \multicolumn{1}{c|}{73.998 $\pm$ 67.546} &
  93.632 $\pm$ 85.124 \\ \midrule
\multicolumn{1}{|c|}{Corr $< 0.5$} &
  \multicolumn{1}{c|}{9.301 $\pm$ 2.655} &
  \multicolumn{1}{c|}{5.179 $\pm$ 2.027} &
  \multicolumn{1}{c|}{0.005 $\pm$ 0.005} &
  \multicolumn{1}{c|}{121.130 $\pm$ 53.542} &
  154.096 $\pm$ 71.022 \\ \midrule
\multicolumn{1}{|c|}{P-Value ($<$ 0.05)} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}0.046} &
  \multicolumn{1}{c|}{0.093} &
  \multicolumn{1}{c|}{0.309} &
  \multicolumn{1}{c|}{0.236} &
  0.381 \\ \midrule
\multicolumn{6}{|l|}{\textbf{TMR5}} \\ \midrule
\multicolumn{1}{|c|}{Corr $\geq 0.5$} &
  \multicolumn{1}{c|}{19.944 $\pm$ 2.810} &
  \multicolumn{1}{c|}{8.550 $\pm$ 2.629} &
  \multicolumn{1}{c|}{0.042 $\pm$ 0.016} &
  \multicolumn{1}{c|}{63.646 $\pm$ 36.385} &
  168.377 $\pm$ 84.488 \\ \midrule
\multicolumn{1}{|c|}{Corr $< 0.5$} &
  \multicolumn{1}{c|}{17.933 $\pm$ 4.627} &
  \multicolumn{1}{c|}{9.514 $\pm$ 2.893} &
  \multicolumn{1}{c|}{0.028 $\pm$ 0.024} &
  \multicolumn{1}{c|}{98.749 $\pm$ 61.789} &
  173.097 $\pm$ 78.176 \\ \midrule
\multicolumn{1}{|c|}{P-Value ($<$ 0.05)} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}0.011} &
  \multicolumn{1}{c|}{0.119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}$<$ 0.05} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}0.017} &
  \cellcolor[HTML]{DAE8FC}0.002 \\ \bottomrule
\end{tabular}

==> TMR1_cluster_45.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{@{}cccccc@{}}
\toprule
 & MFR {[}Hz{]} & Rec Th {[}\% MVC{]} & Territory {[}\%{]} & Amplitude {[}$\mu$V{]} & Size {[}$\muV$ms{]} \\ \midrule
\multicolumn{6}{|c|}{\textbf{TMR1}} \\ \midrule                                                                                                                                  
High corr & 12.934 $\pm$ 2.860 & 6.444 $\pm$ 2.366 & 0.033 $\pm$ 0.047 & 27.986 $\pm$ 27.067 & 55.815 $\pm$ 41.245 \\                     
\hline                                                                                                                                    
Low Corr & 10.600 $\pm$ 3.937 & 9.982 $\pm$ 3.074 & 0.022 $\pm$ 0.034 & 79.680 $\pm$ 99.169 & 154.234 $\pm$ 201.566 \\                    
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.000 & p = 0.267 & p = 0.000 & p = 0.137 \\                                                          
\hline
\hline                                                                                                                                    
High corr & 13.003 $\pm$ 2.748 & 6.381 $\pm$ 2.384 & 0.034 $\pm$ 0.049 & 26.935 $\pm$ 23.171 & 53.668 $\pm$ 32.972 \\                     
\hline                                                                                                                                    
Low Corr & 11.625 $\pm$ 4.150 & 8.641 $\pm$ 2.974 & 0.012 $\pm$ 0.010 & 62.146 $\pm$ 52.928 & 116.944 $\pm$ 102.713 \\                    
\hline                                                                                                                                    
P-Value & p = 0.007 & p = 0.000 & p = 0.019 & p = 0.000 & p = 0.177 \\                                                                    
\hline  
\multicolumn{6}{|c|}{\textbf{TMR3}} \\ \midrule                                                                                                                                  
High corr & 14.685 $\pm$ 4.074 & 5.606 $\pm$ 1.835 & 0.014 $\pm$ 0.030 & 136.709 $\pm$ 100.777 & 144.151 $\pm$ 82.606 \\                  
\hline                                                                                                                                    
Low Corr & 11.691 $\pm$ 5.650 & 5.330 $\pm$ 1.980 & 0.014 $\pm$ 0.029 & 139.442 $\pm$ 95.985 & 185.807 $\pm$ 157.511 \\                   
\hline                                                                                                                                    
P-Value & p = 0.005 & p = 0.489 & p = 0.683 & p = 0.719 & p = 0.861 \\                                                                    
\hline     
\hline                                                                                                                                    
High corr & 14.310 $\pm$ 4.155 & 5.409 $\pm$ 1.837 & 0.014 $\pm$ 0.030 & 132.629 $\pm$ 100.564 & 137.681 $\pm$ 80.274 \\                  
\hline                                                                                                                                    
Low Corr & 11.121 $\pm$ 4.545 & 5.288 $\pm$ 1.895 & 0.019 $\pm$ 0.041 & 139.639 $\pm$ 65.902 & 151.920 $\pm$ 87.966 \\                    
\hline                                                                                                                                    
P-Value & p = 0.046 & p = 0.949 & p = 0.490 & p = 0.435 & p = 0.443 \\                                                                    
\hline  
\multicolumn{6}{|c|}{\textbf{TMR4}} \\ \midrule                                                                                                                                      
High corr & 13.121 $\pm$ 3.892 & 4.310 $\pm$ 1.237 & 0.010 $\pm$ 0.008 & 68.227 $\pm$ 35.513 & 121.447 $\pm$ 84.921 \\                        
\hline                                                                                                                                        
Low Corr & 11.130 $\pm$ 2.889 & 5.828 $\pm$ 1.572 & 0.048 $\pm$ 0.081 & 53.919 $\pm$ 29.653 & 89.000 $\pm$ 44.950 \\                          
\hline                                                                                                                                        
P-Value & p = 0.303 & p = 0.110 & p = 0.696 & p = 0.414 & p = 0.972 \\                                                                        
\hline
\hline                                                                                                                                    
High corr & 12.756 $\pm$ 3.862 & 4.416 $\pm$ 1.057 & 0.010 $\pm$ 0.008 & 70.893 $\pm$ 37.998 & 120.199 $\pm$ 88.903 \\                        
\hline                                                                                                                                        
Low Corr & 13.508 $\pm$ 4.278 & 4.420 $\pm$ 2.009 & 0.012 $\pm$ 0.007 & 62.653 $\pm$ 25.361 & 123.044 $\pm$ 70.819 \\                         
\hline                                                                                                                                        
P-Value & p = 0.861 & p = 0.861 & p = 0.248 & p = 1.000 & p = 0.575 \\                      
\hline
\multicolumn{6}{|c|}{\textbf{TMR5}} \\ \midrule                                                                                                                                  
High corr & 19.900 $\pm$ 3.219 & 8.989 $\pm$ 2.653 & 0.037 $\pm$ 0.019 & 74.628 $\pm$ 47.591 & 166.446 $\pm$ 80.534 \\                    
\hline                                                                                                                                    
Low Corr & 16.441 $\pm$ 4.433 & 10.596 $\pm$ 3.613 & 0.031 $\pm$ 0.023 & 84.679 $\pm$ 51.043 & 168.873 $\pm$ 79.675 \\                    
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.030 & p = 0.064 & p = 0.298 & p = 0.159 \\                                                                    
\hline 
\hline                                                                                                                                 
High corr & 20.150 $\pm$ 3.212 & 8.966 $\pm$ 2.596 & 0.037 $\pm$ 0.019 & 76.725 $\pm$ 47.783 & 167.760 $\pm$ 79.486 \\                    
\hline                                                                                                                                    
Low Corr & 17.933 $\pm$ 3.211 & 9.993 $\pm$ 3.669 & 0.031 $\pm$ 0.017 & 70.288 $\pm$ 44.381 & 150.540 $\pm$ 72.089 \\                     
\hline                                                                                                                                    
P-Value & p = 0.001 & p = 0.173 & p = 0.217 & p = 0.617 & p = 0.808 \\                                                                    
\hline   
\multicolumn{6}{|c|}{\textbf{TMR1}} \\ \midrule     

\hline                                                                                                                                    
High corr & 13.047 $\pm$ 2.726 & 6.309 $\pm$ 2.258 & 0.034 $\pm$ 0.049 & 26.730 $\pm$ 23.850 & 54.563 $\pm$ 39.519 \\                     
\hline                                                                                                                                    
Low Corr & 10.711 $\pm$ 3.962 & 9.718 $\pm$ 3.106 & 0.020 $\pm$ 0.031 & 73.967 $\pm$ 93.491 & 140.385 $\pm$ 186.926 \\                    
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.000 & p = 0.104 & p = 0.000 & p = 0.062 \\                                                                    
\hline
\hline                                                                                                                                    
High corr & 13.153 $\pm$ 2.602 & 6.292 $\pm$ 2.349 & 0.036 $\pm$ 0.052 & 26.795 $\pm$ 24.103 & 55.545 $\pm$ 41.092 \\                     
\hline                                                                                                                                    
Low Corr & 11.138 $\pm$ 3.878 & 8.866 $\pm$ 3.140 & 0.021 $\pm$ 0.028 & 61.667 $\pm$ 83.778 & 116.589 $\pm$ 166.175 \\                    
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.000 & p = 0.379 & p = 0.002 & p = 0.123 \\                                                                    
\hline 
\multicolumn{6}{|c|}{\textbf{TMR3}} \\ \midrule     

\hline                                                                                                                                    
High corr & 14.975 $\pm$ 4.040 & 5.522 $\pm$ 1.774 & 0.015 $\pm$ 0.032 & 134.225 $\pm$ 104.508 & 144.437 $\pm$ 83.007 \\                  
\hline                                                                                                                                    
Low Corr & 12.896 $\pm$ 5.952 & 6.458 $\pm$ 1.943 & 0.007 $\pm$ 0.010 & 164.840 $\pm$ 94.578 & 213.151 $\pm$ 162.901 \\                   
\hline                                                                                                                                    
P-Value & p = 0.072 & p = 0.106 & p = 0.485 & p = 0.132 & p = 0.371 \\                                                                    
\hline 
\hline                                                                                                                                    
High corr & 15.282 $\pm$ 3.755 & 5.466 $\pm$ 1.820 & 0.018 $\pm$ 0.035 & 128.856 $\pm$ 109.284 & 141.458 $\pm$ 83.522 \\                  
\hline                                                                                                                                    
Low Corr & 12.934 $\pm$ 4.804 & 5.767 $\pm$ 1.671 & 0.008 $\pm$ 0.017 & 147.309 $\pm$ 82.169 & 155.626 $\pm$ 85.460 \\                    
\hline                                                                                                                                    
P-Value & p = 0.052 & p = 0.468 & p = 0.127 & p = 0.176 & p = 0.095 \\                                                                    
\hline 
\multicolumn{6}{|c|}{\textbf{TMR4}} \\ \midrule  
\hline                                                                                                                                        
High corr & 13.169 $\pm$ 3.924 & 4.288 $\pm$ 1.314 & 0.010 $\pm$ 0.007 & 69.508 $\pm$ 31.170 & 119.389 $\pm$ 92.181 \\                        
\hline                                                                                                                                        
Low Corr & 13.497 $\pm$ 4.123 & 4.945 $\pm$ 1.796 & 0.013 $\pm$ 0.009 & 51.286 $\pm$ 27.344 & 109.377 $\pm$ 64.702 \\                         
\hline                                                                                                                                        
P-Value & p = 0.973 & p = 0.562 & p = 0.394 & p = 0.094 & p = 0.321 \\                                                                        
\hline   
\hline                                                                                                                                        
High corr & 13.804 $\pm$ 4.401 & 4.131 $\pm$ 1.124 & 0.010 $\pm$ 0.009 & 70.829 $\pm$ 36.140 & 122.399 $\pm$ 100.487 \\                       
\hline                                                                                                                                        
Low Corr & 13.619 $\pm$ 3.806 & 4.103 $\pm$ 1.568 & 0.013 $\pm$ 0.008 & 52.162 $\pm$ 27.065 & 94.971 $\pm$ 74.937 \\                          
\hline                                                                                                                                        
P-Value & p = 1.000 & p = 0.860 & p = 0.375 & p = 0.328 & p = 0.773 \\                                                                        
\hline  
\multicolumn{6}{|c|}{\textbf{TMR5}} \\ \midrule  
\hline                                                                                                                                                                             
High corr & 20.364 $\pm$ 3.030 & 8.627 $\pm$ 2.568 & 0.038 $\pm$ 0.018 & 76.366 $\pm$ 49.649 & 171.176 $\pm$ 81.530 \\                    
\hline                                                                                                                                    
Low Corr & 16.594 $\pm$ 3.917 & 9.588 $\pm$ 3.074 & 0.032 $\pm$ 0.025 & 80.721 $\pm$ 54.354 & 168.379 $\pm$ 83.139 \\                     
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.180 & p = 0.069 & p = 0.895 & p = 0.436 \\                                                                    
\hline 
\hline
High corr & 20.641 $\pm$ 3.112 & 8.282 $\pm$ 2.209 & 0.037 $\pm$ 0.018 & 76.532 $\pm$ 51.205 & 169.607 $\pm$ 82.775 \\                    
\hline                                                                                                                                    
Low Corr & 17.750 $\pm$ 2.534 & 9.452 $\pm$ 3.175 & 0.037 $\pm$ 0.017 & 61.801 $\pm$ 37.196 & 152.749 $\pm$ 72.723 \\                     
\hline                                                                                                                                    
P-Value & p = 0.000 & p = 0.084 & p = 0.933 & p = 0.266 & p = 0.317 \\                                                                    
\hline
\end{tabular}

==> protocol-tab.tex <==
\begin{tabular}{@{}llll@{}}
\toprule
{\color[HTML]{333333} \textbf{TMR volunteers}} &
  {\color[HTML]{333333} \textbf{P1}} &
  {\color[HTML]{333333} \textbf{P2}} &
  {\color[HTML]{333333} \textbf{P3}} \\ \midrule
\rowcolor[HTML]{E1E4E9} 
{\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}l@{}}TMR site and nerve\\ \\ \end{tabular}}} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Pectoral major clavicular part - Ulnar\\ Pectoral major sternocostal part - Median\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Biceps short head - Ulnar\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Pectoral minor - Ulnar\\ Latissimus dorsi - Radial\end{tabular}} \\
\textbf{\begin{tabular}[c]{@{}l@{}}Insertion location -\\ microelectrode 1\end{tabular}} &
  Pectoral major clavicular part - Ulnar &
  Biceps short head - Ulnar &
  Pectoral minor  - Ulnar \\
\rowcolor[HTML]{E1E4E9} 
\textbf{\begin{tabular}[c]{@{}l@{}}Movements associated \\ with microelectrode 1\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Ulnar deviation\\ Pinky flexion\\ Pinky abduction\\ Intrinsic position (MCP flexion)\\ Fist/flexion of fingers\\ Wrist flexion\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Ulnar deviation (-) Pinky flexion  Intrinsic and thumb adduction  Fist/flexion of fingers  \end{tabular}}&
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Ulnar deviation*\\ Pinky flexion\\ Pinky abduction* \\ Intrinsic position (MCP flexion) \\ Thumb adduction\\ \\ \end{tabular}} \\
\textbf{\begin{tabular}[c]{@{}l@{}}Insertion location -\\ microelectrode 2\end{tabular}} &
  Pectoral major sternocostal part - Median &
  &
  Latissimus dorsi - Radial \\
\rowcolor[HTML]{E1E4E9} 
\textbf{\begin{tabular}[c]{@{}l@{}}Movements associated \\ with microelectrode 2\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Wrist flexion\\ Pronation\\ Thumb opposition\\ Tripod grip\\ Fist/flexion of fingers\\ \\ \end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}   \end{tabular}}&
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Supination\\ Wrist extension (-)\\ Finger extension\\ Thumb extension\\ Index finger extension (-)\\ Pinky extension\end{tabular}} \\
{\color[HTML]{333333} \textbf{Protocol}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}4 reps per movement, \\ Ramps: 4 s\\ Isometric: 10 sec at 10\% MVC\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}6 reps per movement\\ Ramps: 2 s\\ Isometric: 5 s at 20\% MVC\end{tabular}} &
  {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}6 reps per movement, \\ Ramps: 2 s\\ Isometric: 5 s at 10\% MVC\\   \\ * Ramp: 4 s \\  Isometric: 5 s at 20\% MVC\end{tabular}} \\ \bottomrule
\end{tabular}%

==> regression-tab.tex <==
\begin{tabular}{@{}llllllllllllllll@{}}
\toprule
\multicolumn{4}{c}{TMR1} &
  \multicolumn{4}{c}{TMR3} &
  \multicolumn{4}{c}{TMR4} &
  \multicolumn{4}{c}{TMR5} \\ \midrule
\multicolumn{16}{|c|}{Recruitment threshold - Average Firing Rate} \\ \midrule
\multicolumn{1}{|l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} \\ \midrule
\multicolumn{1}{|l|}{Wrist Flexion} &
  \multicolumn{1}{l|}{0.22} &
  \multicolumn{1}{l|}{9.26} &
  \multicolumn{1}{l|}{0.07} &
  \multicolumn{1}{l|}{Flexion of Fingers} &
  \multicolumn{1}{l|}{-0.7} &
  \multicolumn{1}{l|}{21.06} &
  \multicolumn{1}{l|}{0.11} &
  \multicolumn{1}{l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{-1.15} &
  \multicolumn{1}{l|}{17.84} &
  \multicolumn{1}{l|}{0.4} &
  \multicolumn{1}{l|}{Index Extension} &
  \multicolumn{1}{l|}{0.32} &
  \multicolumn{1}{l|}{15.56} &
  \multicolumn{1}{l|}{0.11} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{-0.15} &
  \multicolumn{1}{l|}{13.17} &
  \multicolumn{1}{l|}{0.03} &
  \multicolumn{1}{l|}{Tripod} &
  \multicolumn{1}{l|}{-0.03} &
  \multicolumn{1}{l|}{10.87} &
  \multicolumn{1}{l|}{0} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Pinky Extension} &
  \multicolumn{1}{l|}{-0.13} &
  \multicolumn{1}{l|}{21.14} &
  \multicolumn{1}{l|}{0.07} \\ \cmidrule(r){1-8} \cmidrule(l){13-16} 
\multicolumn{1}{|l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{-0.47} &
  \multicolumn{1}{l|}{18.52} &
  \multicolumn{1}{l|}{0.24} &
  \multicolumn{1}{l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{-2.91} &
  \multicolumn{1}{l|}{27.87} &
  \multicolumn{1}{l|}{0.45} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Thumb Extension} &
  \multicolumn{1}{l|}{-3.36} &
  \multicolumn{1}{l|}{48.21} &
  \multicolumn{1}{l|}{0.7} \\ \cmidrule(r){1-8} \cmidrule(l){13-16} 
\multicolumn{1}{|l|}{Pinky Abduction} &
  \multicolumn{1}{l|}{-0.78} &
  \multicolumn{1}{l|}{16.43} &
  \multicolumn{1}{l|}{0.58} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Intrinsic} &
  \multicolumn{1}{l|}{-0.62} &
  \multicolumn{1}{l|}{16.12} &
  \multicolumn{1}{l|}{0.16} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Tripod} &
  \multicolumn{1}{l|}{-1.95} &
  \multicolumn{1}{l|}{24.93} &
  \multicolumn{1}{l|}{0.87} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{16}{|c|}{Recruitment threshold - Derecruitment threshold} \\ \midrule
\multicolumn{1}{|l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} \\ \midrule
\multicolumn{1}{|l|}{Wrist Flexion} &
  \multicolumn{1}{l|}{0.01} &
  \multicolumn{1}{l|}{9.26} &
  \multicolumn{1}{l|}{0} &
  \multicolumn{1}{l|}{Flexion of Fingers} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.18} &
  \multicolumn{1}{l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{0.21} &
  \multicolumn{1}{l|}{4.05} &
  \multicolumn{1}{l|}{0.37} &
  \multicolumn{1}{l|}{Index Extension} &
  \multicolumn{1}{l|}{0.16} &
  \multicolumn{1}{l|}{8.17} &
  \multicolumn{1}{l|}{0.01} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{-0.75} &
  \multicolumn{1}{l|}{10.51} &
  \multicolumn{1}{l|}{0.48} &
  \multicolumn{1}{l|}{Tripod} &
  \multicolumn{1}{l|}{0.92} &
  \multicolumn{1}{l|}{1.83} &
  \multicolumn{1}{l|}{0.94} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Pinky Extension} &
  \multicolumn{1}{l|}{0.71} &
  \multicolumn{1}{l|}{2.26} &
  \multicolumn{1}{l|}{0.86} \\ \midrule
\multicolumn{1}{|l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{-0.67} &
  \multicolumn{1}{l|}{15.7} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{0.7} &
  \multicolumn{1}{l|}{2.03} &
  \multicolumn{1}{l|}{0.49} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Thumb Extension} &
  \multicolumn{1}{l|}{-3.56} &
  \multicolumn{1}{l|}{40.81} &
  \multicolumn{1}{l|}{0.79} \\ \midrule
\multicolumn{1}{|l|}{Pinky Abduction} &
  \multicolumn{1}{l|}{0.05} &
  \multicolumn{1}{l|}{4.75} &
  \multicolumn{1}{l|}{0} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Intrinsic} &
  \multicolumn{1}{l|}{0.24} &
  \multicolumn{1}{l|}{5.73} &
  \multicolumn{1}{l|}{0.05} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Tripod} &
  \multicolumn{1}{l|}{0.74} &
  \multicolumn{1}{l|}{2.85} &
  \multicolumn{1}{l|}{0.54} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \midrule
\multicolumn{16}{|c|}{Recruitment threshold - MUAP size} \\ \midrule
\multicolumn{1}{|l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} &
  \multicolumn{1}{l|}{Task} &
  \multicolumn{1}{l|}{Slope} &
  \multicolumn{1}{l|}{Intercept} &
  \multicolumn{1}{l|}{$R^{2}$} \\ \midrule
\multicolumn{1}{|l|}{Wrist Flexion} &
  \multicolumn{1}{l|}{25.91} &
  \multicolumn{1}{l|}{-145.6} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{Flexion of Fingers} &
  \multicolumn{1}{l|}{7.43} &
  \multicolumn{1}{l|}{167.89} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{-5.56} &
  \multicolumn{1}{l|}{142.64} &
  \multicolumn{1}{l|}{0.01} &
  \multicolumn{1}{l|}{Index Extension} &
  \multicolumn{1}{l|}{10.13} &
  \multicolumn{1}{l|}{102.74} &
  \multicolumn{1}{l|}{0.21} \\ \midrule
\multicolumn{1}{|l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{10.45} &
  \multicolumn{1}{l|}{-14.03} &
  \multicolumn{1}{l|}{0.64} &
  \multicolumn{1}{l|}{Tripod} &
  \multicolumn{1}{l|}{88.76} &
  \multicolumn{1}{l|}{-277.85} &
  \multicolumn{1}{l|}{0.91} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Pinky Extension} &
  \multicolumn{1}{l|}{21.70} &
  \multicolumn{1}{l|}{-39.26} &
  \multicolumn{1}{l|}{0.79} \\ \cmidrule(r){1-8} \cmidrule(l){13-16} 
\multicolumn{1}{|l|}{Pinky Flexion} &
  \multicolumn{1}{l|}{16.21} &
  \multicolumn{1}{l|}{-65.94} &
  \multicolumn{1}{l|}{0.28} &
  \multicolumn{1}{l|}{Ulnar Deviation} &
  \multicolumn{1}{l|}{-63.9} &
  \multicolumn{1}{l|}{422.65} &
  \multicolumn{1}{l|}{0.81} &
   &
   &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{Thumb Extension} &
  \multicolumn{1}{l|}{-38.72} &
  \multicolumn{1}{l|}{482.76} &
  \multicolumn{1}{l|}{0.1} \\ \cmidrule(r){1-8} \cmidrule(l){13-16} 
\multicolumn{1}{|l|}{Pinky Abduction} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{70.16} &
  \multicolumn{1}{l|}{0} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Intrinsic} &
  \multicolumn{1}{l|}{42.65} &
  \multicolumn{1}{l|}{-206.94} &
  \multicolumn{1}{l|}{0.62} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\multicolumn{1}{|l|}{Tripod} &
  \multicolumn{1}{l|}{2.64} &
  \multicolumn{1}{l|}{11.72} &
  \multicolumn{1}{l|}{0.03} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-4}
\end{tabular}

==> sharedunits.tex <==

\begin{table}
    \centering
    \begin{tabular}{cccc}
         TMR1&  # Shared MUs&  # Independent MUs& # Total\\
         Wrist Flexion&  6&  1& 7\\
         Ulnar Deviation&  3&  5& 8\\
         Pinky Flexion&  4&  4& 8\\
         Pinky Abduction&  4&  4& 8\\
         Intrinsic&  4&  3& 7\\
         Tripod&  3&  6& 9\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
